Counterfactual Invariance to Spurious Correlations: Why and How to Pass Stress Tests

Informally, a 'spurious correlation' is the dependence of a model on some aspect of the input data that an analyst thinks shouldn't matter. In machine learning, these have a know-it-when-you-see-it character; e.g., changing the gender of a sentence's subject changes a sentiment predictor's output. To check for spurious correlations, we can 'stress test' models by perturbing irrelevant parts of input data and seeing if model predictions change. In this paper, we study stress testing using the tools of causal inference. We introduce counterfactual invariance as a formalization of the requirement that changing irrelevant parts of the input shouldn't change model predictions. We connect counterfactual invariance to out-of-domain model performance, and provide practical schemes for learning (approximately) counterfactual invariant predictors (without access to counterfactual examples). It turns out that both the means and implications of counterfactual invariance depend fundamentally on the true underlying causal structure of the data -- in particular, whether the label causes the features or the features cause the label. Distinct causal structures require distinct regularization schemes to induce counterfactual invariance. Similarly, counterfactual invariance implies different domain shift guarantees depending on the underlying causal structure. This theory is supported by empirical results on text classification.

==> figures/bonus-figures.tex <==
\begin{tikzpicture}[var/.style={draw,circle,inner sep=0pt,minimum size=1.2cm}]
    % Nodes
    \node (Z) [var] {$Z$};
    \node (X) [var, right=.8cm of Z] {$X$};
    \node (Y) [var, right=.8cm of X] {$Y$};
    
    % Arrows
    \path[->, line width=0.5mm]
        (Z) edge (X)
        (X) edge (Y);
    \path[<->]
    (Z) edge[bend right=90, line width=0.5mm, looseness=1.5, dashed] (Y);
\end{tikzpicture}

\vspace{2cm}

\begin{tikzpicture}[var/.style={draw,circle,inner sep=0pt,minimum size=1.2cm}]
    % Nodes
    \node (Y) [var] {$Y$};
    \node (Z) [var, below=1cm of Y] {$Z$};
    \node (X) [var, right=2cm of Y, below=0.5cm of Y] {$X$};
    % Arrows
    \path[->, line width=0.5mm]
        (Z) edge (X)
        (Y) edge (X);
    \path[<->, line width=0.5mm]
    (Z) edge[bend left=90, dashed] (Y);
\end{tikzpicture}

\vspace{2cm}

\begin{tikzpicture}[
var/.style={draw,circle,inner sep=0pt,minimum size=1.2cm},
latentconf/.style={draw,circle,dashed,inner sep=0pt,minimum size=1.2cm, fill=green!5}
]
    % Nodes
    \node (Z) [var] {$Z$};
    \node (Xyz) [var, right=.8cm of Z] {$\xyz$};
    \node (Xzperp) [var, above=0.25cm of Xyz] {$\xy$};
    \node (Xyperp) [var, below=0.25cm of Xyz] {$\xz$};
    \node (Y) [var, right=.8cm of Xyz] {$Y$};
    \node (U) [latentconf, left=.8cm of Z] {$U$};
    % Arrows
    \path[->, line width=0.5mm]
        (U) edge[bend right=90, looseness=1.25] (Y)
        (U) edge (Z)
        (Z) edge (Xyz)
            edge (Xyperp)
        (Xyz) edge (Y)
              edge (Xyperp)
        (Xzperp) edge (Y)
                 edge (Xyz);
\end{tikzpicture}

\vspace{2cm}

\begin{tikzpicture}[
var/.style={draw,circle,inner sep=0pt,minimum size=1.2cm},
latentconf/.style={draw,circle,dashed,inner sep=0pt,minimum size=1.2cm, fill=green!5}
]
    % Nodes
    \node (Y) [var] {$Y$};
    \node (Z) [var, below=1cm of Y] {$Z$};
    \node (Xzperp) [var, right=1cm of Y] {$\xy$};
    \node (Xyz) [var, below=0.2cm of Xzperp] {$\xyz$};
    \node (Xyperp) [var, below=0.2cm of Xyz] {$\xz$};
    \node (U) [latentconf, left=0.8cm of Z] {$U$};
    % Arrows
    \path[->, line width=0.5mm]
        (U) edge (Y)
            edge (Z)
        (Z) edge (Xyz)
            edge (Xyperp)
        (Y) edge (Xyz)
        (Y) edge (Xzperp)
        (Xzperp) edge (Xyz)
        (Xyperp) edge (Xyz);
\end{tikzpicture}

==> on-perturbative-stress-testing/figures/bonus-figures.tex <==
\begin{tikzpicture}[var/.style={draw,circle,inner sep=0pt,minimum size=1.2cm}]
    % Nodes
    \node (Z) [var] {$Z$};
    \node (X) [var, right=.8cm of Z] {$X$};
    \node (Y) [var, right=.8cm of X] {$Y$};
    
    % Arrows
    \path[->, line width=0.5mm]
        (Z) edge (X)
        (X) edge (Y);
    \path[<->]
    (Z) edge[bend right=90, line width=0.5mm, looseness=1.5, dashed] (Y);
\end{tikzpicture}

\vspace{2cm}

\begin{tikzpicture}[var/.style={draw,circle,inner sep=0pt,minimum size=1.2cm}]
    % Nodes
    \node (Y) [var] {$Y$};
    \node (Z) [var, below=1cm of Y] {$Z$};
    \node (X) [var, right=2cm of Y, below=0.5cm of Y] {$X$};
    % Arrows
    \path[->, line width=0.5mm]
        (Z) edge (X)
        (Y) edge (X);
    \path[<->, line width=0.5mm]
    (Z) edge[bend left=90, dashed] (Y);
\end{tikzpicture}

\vspace{2cm}

\begin{tikzpicture}[
var/.style={draw,circle,inner sep=0pt,minimum size=1.2cm},
latentconf/.style={draw,circle,dashed,inner sep=0pt,minimum size=1.2cm, fill=green!5}
]
    % Nodes
    \node (Z) [var] {$Z$};
    \node (Xyz) [var, right=.8cm of Z] {$\xyz$};
    \node (Xzperp) [var, above=0.25cm of Xyz] {$\xy$};
    \node (Xyperp) [var, below=0.25cm of Xyz] {$\xz$};
    \node (Y) [var, right=.8cm of Xyz] {$Y$};
    \node (U) [latentconf, left=.8cm of Z] {$U$};
    % Arrows
    \path[->, line width=0.5mm]
        (U) edge[bend right=90, looseness=1.25] (Y)
        (U) edge (Z)
        (Z) edge (Xyz)
            edge (Xyperp)
        (Xyz) edge (Y)
              edge (Xyperp)
        (Xzperp) edge (Y)
                 edge (Xyz);
\end{tikzpicture}

\vspace{2cm}

\begin{tikzpicture}[
var/.style={draw,circle,inner sep=0pt,minimum size=1.2cm},
latentconf/.style={draw,circle,dashed,inner sep=0pt,minimum size=1.2cm, fill=green!5}
]
    % Nodes
    \node (Y) [var] {$Y$};
    \node (Z) [var, below=1cm of Y] {$Z$};
    \node (Xzperp) [var, right=1cm of Y] {$\xy$};
    \node (Xyz) [var, below=0.2cm of Xzperp] {$\xyz$};
    \node (Xyperp) [var, below=0.2cm of Xyz] {$\xz$};
    \node (U) [latentconf, left=0.8cm of Z] {$U$};
    % Arrows
    \path[->, line width=0.5mm]
        (U) edge (Y)
            edge (Z)
        (Z) edge (Xyz)
            edge (Xyperp)
        (Y) edge (Xyz)
        (Y) edge (Xzperp)
        (Xzperp) edge (Xyz)
        (Xyperp) edge (Xyz);
\end{tikzpicture}

==> on-perturbative-stress-testing/figures/scm-anticausal.tex <==
\begin{tikzpicture}[var/.style={draw,circle,inner sep=0pt,minimum size=1.2cm}]
    % Nodes
    \node (Y) [var] {$Y$};
    \node (Z) [var, below=1cm of Y] {$Z$};
    \node (Xzperp) [var, right=1cm of Y] {$\xy$};
    \node (Xyz) [var, below=0.2cm of Xzperp] {$\xyz$};
    \node (Xyperp) [var, below=0.2cm of Xyz] {$\xz$};
    
    % Arrows
    \path[->]
        (Z) edge (Xyz)
            edge (Xyperp)
        (Y) edge (Xyz)
        (Y) edge (Xzperp)
        (Xzperp) edge (Xyz)
        (Xyperp) edge (Xyz);
    \path[<->]
    (Z) edge[bend left=90, dashed] (Y);
\end{tikzpicture}

==> on-perturbative-stress-testing/figures/scm-causal.tex <==
\begin{tikzpicture}[var/.style={draw,circle,inner sep=0pt,minimum size=1.2cm}]
    % Nodes
    \node (Z) [var] {$Z$};
    \node (Xyz) [var, right=.8cm of Z] {$\xyz$};
    \node (Xzperp) [var, above=0.25cm of Xyz] {$\xy$};
    \node (Xyperp) [var, below=0.25cm of Xyz] {$\xz$};
    \node (Y) [var, right=.8cm of Xyz] {$Y$};
    
    % Arrows
    \path[->]
        (Z) edge (Xyz)
            edge (Xyperp)
        (Xyz) edge (Y)
              edge (Xyperp)
        (Xzperp) edge (Y)
                 edge (Xyz);
    \path[<->]
    (Z) edge[bend right=90, looseness=1.5, dashed] (Y);
\end{tikzpicture}

==> on-perturbative-stress-testing/preamble/commenting.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% EDITING HELPER FUNCTIONS  %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% NA: needs attention (rough writing whose correctness needs to be verified)
%% TBD: instructions for how to fix a gap ("Describe the propagation by ...")
%% PROBLEM: bug or missing crucial bit 

%% use \fXXX versions of these macros to put additional explanation into a footnote.  
%% The idea is that we don't want to interrupt the flow of the paper or make it 
%% impossible to read because there are a bunch of comments.

%% NA's (and TBDs, those less crucially) should be written so 
%% that they flow with the text.

\definecolor{WowColor}{rgb}{.75,0,.75}
\definecolor{SubtleColor}{rgb}{0,0,.50}

% inline
\newcommand{\NA}[1]{\textcolor{SubtleColor}{ {\tiny \bf ($\star$)} #1}}
\newcommand{\LATER}[1]{\textcolor{SubtleColor}{ {\tiny \bf ($\dagger$)} #1}}
\newcommand{\TBD}[1]{\textcolor{SubtleColor}{ {\tiny \bf (!)} #1}}
\newcommand{\PROBLEM}[1]{\textcolor{WowColor}{ {\bf (!!)} {\bf #1}}}

% as margin notes

\newcounter{margincounter}
\newcommand{\displaycounter}{{\arabic{margincounter}}}
\newcommand{\incdisplaycounter}{{\stepcounter{margincounter}\arabic{margincounter}}}

\newcommand{\fTBD}[1]{\textcolor{SubtleColor}{$\,^{(\incdisplaycounter)}$}\marginpar{\tiny\textcolor{SubtleColor}{ {\tiny $(\displaycounter)$} #1}}}

\newcommand{\fPROBLEM}[1]{\textcolor{WowColor}{$\,^{((\incdisplaycounter))}$}\marginpar{\tiny\textcolor{WowColor}{ {\bf $\mathbf{((\displaycounter))}$} {\bf #1}}}}

\newcommand{\fLATER}[1]{\textcolor{SubtleColor}{$\,^{(\incdisplaycounter\dagger)}$}\marginpar{\tiny\textcolor{SubtleColor}{ {\tiny $(\displaycounter\dagger)$} #1}}}


==> on-perturbative-stress-testing/preamble/definitions_basic.tex <==
% This file contains definitions of custom macros
% ------------------------------------------------------------------------------

\newcommand{\defnphrase}[1]{\emph{#1}}

\global\long\def\floor#1{\lfloor#1\rfloor}

%\newcommand{\st}{\,:\,}
\newcommand{\defeq}{\coloneqq}
\newcommand{\asympeq}{\ \sim\ }

\newcommand{\Reals}{\mathbb{R}}
\newcommand{\Nats}{\mathbb{N}}
\newcommand{\NNReals}{\Reals_{+}}


\newcommand{\exclude}{\backslash}

\newcommand{\eps}{\varepsilon}

\renewcommand{\Re}{\mathrm{Re}}
\renewcommand{\Im}{\mathrm{Im}}

\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\logit}{logit}


% Graph theory
\newcommand{\edges}{e}
\newcommand{\vertices}{v}
\newcommand{\loops}{l}


% Probability
\newcommand{\EE}{\mathbb{E}}
\newcommand{\var}{\mathrm{var}}
\renewcommand{\Pr}{\mathrm{P}}
\newcommand{\convPr}{\xrightarrow{\,p\,}}
\newcommand{\convDist}{\xrightarrow{\,d\,}}
\newcommand{\equaldist}{\overset{d}{=}}
\newcommand{\upto}{\!\uparrow\!}
\newcommand{\given}{\mid}
\newcommand{\st}{:}
\newcommand{\as}{\textrm{ a.s.}}
\newcommand{\equalas}{\overset{\mathrm{a.s.}}{=}}
\newcommand{\abs}[1]{\left\lvert#1 \right\rvert}
\newcommand{\intd}{\mathrm{d}}
\newcommand{\dist}{\ \sim\ }
\newcommand{\distiid}{\overset{\mathrm{iid}}{\dist}}
\newcommand{\distind}{\overset{ind}{\dist}}
\newcommand{\dtv}[1]{\|#1\|_{\mathrm{TV}}}
%\newcommand{\PP}{\Pi}
\newcommand{\PPDist}{\mathrm{PP}}

\newcommand{\Lebesgue}{\Lambda}
\newcommand{\NatSubs}[1]{\tilde \Nats_{#1}}

% Causality
\newcommand{\cdo}{\mathrm{do}} 

% Distributions
\newcommand{\normalDist}{\mathrm{Normal}}
\newcommand{\diriDist}{\mathrm{Diri}}
\newcommand{\categDist}{\mathrm{Cat}}
\newcommand{\betaDist}{\mathrm{Beta}}
\newcommand{\bernDist}{\mathrm{Bern}}
\newcommand{\binDist}{\mathrm{Bin}}
\newcommand{\uniDist}{\mathrm{Uni}}
\newcommand{\poiDist}{\mathrm{Poi}}
\newcommand{\gammaDist}{\mathrm{Gamma}}
\newcommand{\multiDist}{\mathrm{Multi}}


% \Set command
\providecommand\given{} % so it exists
\newcommand\SetSymbol[1][]{
  \nonscript\,#1:\nonscript\,\mathopen{}\allowbreak}
\DeclarePairedDelimiterX\Set[1]{\lbrace}{\rbrace}%
{ \renewcommand\given{\SetSymbol[]} #1 }

% Indicator
\newcommand{\Ind}{\mathbbm{1}}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> on-perturbative-stress-testing/preamble/minimalist_biblatex.tex <==
\usepackage[%
minnames=1,maxnames=99,maxcitenames=2,
style=alphabetic,
doi=false,
url=false,
firstinits=true,
hyperref,
natbib,
backend=bibtex,
sorting=nyt
]{biblatex}%

\newbibmacro*{journal}{%
  \iffieldundef{journaltitle}
    {}
    {\printtext[journaltitle]{%
       \printfield[noformat]{journaltitle}%
       \setunit{\subtitlepunct}%
       \printfield[noformat]{journalsubtitle}}}}

%\DeclareFieldFormat[article,inbook,incollection,inproceedings,patent,thesis,unpublished]{titlecase}{\MakeSentenceCase*{#1}}
% print the title of articles and any in* type entry in sentence case
\DeclareFieldFormat{sentencecase}{\MakeSentenceCase*{#1}}

\renewbibmacro*{title}{%
  \ifthenelse{\iffieldundef{title}\AND\iffieldundef{subtitle}}
    {}
    {\ifthenelse{\ifentrytype{article}\OR\ifentrytype{inbook}%
      \OR\ifentrytype{incollection}\OR\ifentrytype{inproceedings}%
      \OR\ifentrytype{inreference}}
      {\printtext[title]{%
        \printfield[sentencecase]{title}%
        \setunit{\subtitlepunct}%
        \printfield[sentencecase]{subtitle}}}%
      {\printtext[title]{%
        \printfield[titlecase]{title}%
        \setunit{\subtitlepunct}%
        \printfield[titlecase]{subtitle}}}%
     \newunit}%
  \printfield{titleaddon}}



\AtEveryBibitem{%
\ifentrytype{article}{
    \clearfield{url}%
    \clearfield{urldate}%
%    \clearfield{eprint}
    \clearfield{eid}
}{}
\ifentrytype{book}{
    \clearfield{url}%
    \clearfield{urldate}%
}{}
\ifentrytype{collection}{
    \clearfield{url}%
    \clearfield{urldate}%
}{}
\ifentrytype{incollection}{
    \clearfield{url}%
    \clearfield{urldate}%
}{}
}

\AtEveryBibitem{
    \clearfield{pages}
    \clearfield{review}%
    \clearfield{series}%%
    \clearfield{volume}
    \clearfield{month}
%    \clearfield{eprint}
    \clearfield{isbn}
    \clearfield{issn}
    \clearlist{location}
    \clearfield{series}
    \clearlist{publisher}
    \clearname{editor}
}{}

==> on-perturbative-stress-testing/preamble/nocommenting.tex <==
\newcommand{\LATER}[1]{\error}
\newcommand{\fLATER}[1]{\error}
\newcommand{\TBD}[1]{\error}
\newcommand{\fTBD}[1]{}
\newcommand{\PROBLEM}[1]{\error}
\newcommand{\fPROBLEM}[1]{\error}
\newcommand{\NA}[1]{#1} 


==> on-perturbative-stress-testing/preamble/preamble.tex <==
%\RequirePackage[l2tabu, orthodox]{nag}

% FONTS
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts

% Replace default Latin Modern typewriter with its proportional counterpart
% http://www.tug.dk/FontCatalogue/lmoderntypewriterprop/
\renewcommand*\ttdefault{lmvtt}


%%% OPTION 1 - Fourier Math + New Century Schoolbook + ParaType Sans

% % Import Fourier Math (this imposes its own New Century Schoolbook type)
% % http://www.ctan.org/tex-archive/fonts/fouriernc/
% \usepackage{fouriernc}
% \usepackage{amsmath}
% % Replace with TeX Gyre Schola version of New Century Schoolbook (must scale!)
% % http://www.tug.dk/FontCatalogue/tgschola/
% \usepackage[scale=0.92]{tgschola}
% \usepackage[scaled=0.88]{PTSans}

%% OPTION 2 - MathDesign Math + Bitstream Charter + ParaType Sans

% Import MathDesign (this brings along Bitstream Charter)
% http://www.ctan.org/tex-archive/fonts/mathdesign/
\usepackage[bitstream-charter]{mathdesign}
\usepackage{amsmath}
\usepackage[scaled=0.92]{PTSans}


% %%% OPTION 3 - MTPRO 2 Math + Termes Times + ParaType Sans

% \usepackage{tgtermes}
% \usepackage{amsmath}
% \usepackage[subscriptcorrection,
%             amssymbols,
%             mtpbb,
%             mtpcal,
%             nofontinfo  % suppresses all warnings
%            ]{mtpro2}
% \usepackage{scalefnt,letltxmacro}
% \LetLtxMacro{\oldtextsc}{\textsc}
% \renewcommand{\textsc}[1]{\oldtextsc{\scalefont{1.10}#1}}
% \usepackage[scaled=0.92]{PTSans}

% GEOMETRY
\usepackage[
  paper  = letterpaper,
  left   = 1.65in,
  right  = 1.65in,
  top    = 1.0in,
 bottom = 1.0in,
 ]{geometry}

% COLOR
\usepackage[usenames,dvipsnames,table]{xcolor}
%\usepackage[usenames,table]{xcolor}
\definecolor{shadecolor}{gray}{0.9}

% SPACING and TEXT
\usepackage[final,expansion=alltext]{microtype}
\usepackage[english]{babel}
\usepackage[parfill]{parskip}
\usepackage{afterpage}
\usepackage{framed}

% tikz
\usepackage{pgf,tikz}
\usetikzlibrary{positioning}


%redefine the leftbar environment to accept a width and coloring options
\renewenvironment{leftbar}[1][\hsize]
{%
  \def\FrameCommand
  {%
    {\color{Gray}\vrule width 3pt}%
    \hspace{10pt}%
    %\hspace{0pt}\fboxsep=\FrameSep\colorbox{black!10}%
  }%
  \MakeFramed{\hsize#1\advance\hsize-\width\FrameRestore}%
}%
{\endMakeFramed}

% define a paragraph header function
\DeclareRobustCommand{\parhead}[1]{\textbf{#1}~}

% EDITING
% line numbering in left margin
\usepackage{lineno}
\renewcommand\linenumberfont{\normalfont
                             \footnotesize
                             \sffamily
                             \color{SkyBlue}}
% ragged paragraphs in right margin
\usepackage{ragged2e}
\DeclareRobustCommand{\sidenote}[1]{\marginpar{
                                    \RaggedRight
                                    \textcolor{Plum}{\textsf{#1}}}}
% paragraph counter in right margin
\newcommand{\parnum}{\bfseries\P\arabic{parcount}}
\newcounter{parcount}
\newcommand\p{%
    \stepcounter{parcount}%
    \leavevmode\marginpar[\hfill\parnum]{\parnum}%
}
% paragraph helper
\DeclareRobustCommand{\PP}{\textcolor{Plum}{\P} }

% COUNTERS
\renewcommand{\labelenumi}{\color{black!67}{\arabic{enumi}.}}
\renewcommand{\labelenumii}{{\color{black!67}(\alph{enumii})}}
\renewcommand{\labelitemi}{{\color{black!67}\textbullet}}

% FIGURES
\usepackage{graphicx}
\usepackage{wrapfig}
\usepackage[labelfont=bf,font=footnotesize,width=.9\textwidth]{caption}
\usepackage[format=hang]{subcaption}

% TABLES
\usepackage{booktabs,multirow,multicol}       % professional-quality tables

% ALGORITHMS
\usepackage[algoruled]{algorithm2e}
\usepackage{listings}
\usepackage{fancyvrb}
\fvset{fontsize=\normalsize}

% BIBLIOGRAPHY
%\usepackage{natbib}

% HYPERREF
\usepackage[colorlinks,linktoc=all]{hyperref}
\usepackage[all]{hypcap}
\hypersetup{citecolor=MidnightBlue}
\hypersetup{linkcolor=MidnightBlue}
\hypersetup{urlcolor=MidnightBlue}

% CLEVEREF must come after HYPERREF
\usepackage[nameinlink]{cleveref}

% ACRONYMS
\usepackage[acronym,smallcaps,nowarn]{glossaries}
% \makeglossaries

% COLOR DEFINITIONS
\newcommand{\red}[1]{\textcolor{BrickRed}{#1}}
\newcommand{\orange}[1]{\textcolor{BurntOrange}{#1}}
\newcommand{\green}[1]{\textcolor{OliveGreen}{#1}}
\newcommand{\blue}[1]{\textcolor{MidnightBlue}{#1}}
\newcommand{\gray}[1]{\textcolor{black!60}{#1}}

% LISTINGS DEFINTIONS
\lstdefinestyle{mystyle}{
    commentstyle=\color{OliveGreen},
    keywordstyle=\color{BurntOrange},
    numberstyle=\tiny\color{black!60},
    stringstyle=\color{MidnightBlue},
    basicstyle=\ttfamily,
    breakatwhitespace=false,
    breaklines=true,
    captionpos=b,
    keepspaces=true,
    numbers=left,
    numbersep=5pt,
    showspaces=false,
    showstringspaces=false,
    showtabs=false,
    tabsize=2
}
\lstset{style=mystyle}


==> on-perturbative-stress-testing/preamble/preamble_math.tex <==
% !TEX root = main.tex


\usepackage{centernot}
\usepackage{amsthm}
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{mathtools}
\usepackage{amsbsy}
\usepackage{amstext}
\usepackage{amsthm}
%\usepackage{amssymb}
\usepackage{thmtools}
\usepackage{thm-restate}

% compatibility w/ parskip https://tex.stackexchange.com/questions/25346/wrong-spacing-before-theorem-environment-amsthm
% \begingroup
%     \makeatletter
%     \@for\theoremstyle:=definition,remark,plain\do{%
%         \expandafter\g@addto@macro\csname th@\theoremstyle\endcsname{%
%             \addtolength\thm@preskip\parskip
%             }%
%         }
% \endgroup

\DeclareRobustCommand{\mb}[1]{\ensuremath{\mathbf{\boldsymbol{#1}}}}
% \DeclareRobustCommand{\mb}[1]{\mathbold{#1}}

\DeclareRobustCommand{\KL}[2]{\ensuremath{\textrm{KL}\left(#1\;\|\;#2\right)}}

% \DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\argmin}{arg\,min}

\crefname{lemma}{lemma}{lemmas}
\Crefname{lemma}{Lemma}{Lemmas}
\crefname{thm}{theorem}{theorems}
\Crefname{thm}{Theorem}{Theorems}
\crefname{prop}{proposition}{propositions}
\Crefname{prop}{Proposition}{Propositions}
\crefname{assumption}{assumption}{assumptions}
\crefname{assumption}{Assumption}{Assumptions}


% \newtheorem{thm}{Theorem} % reset theorem numbering for each chapter
% \newtheorem{defn}{Definition} % definition numbers are dependent on theorem numbers
% \newtheorem{prop}[thm]{Proposition}
% \newtheorem{exmp}[thm]{Example} % same for example numbers
% \newtheorem{lemma}[thm]{Lemma}
% \newtheorem{assumption}{Assumption}
% \newtheorem{corollary}[thm]{Corollary}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}
\newcommand{\independent}{\protect\mathpalette{\protect\independenT}{\perp}}

\newcommand{\grad}{\nabla}

\renewcommand{\mid}{~\vert~}
\newcommand{\prm}{\:;\:}

\newcommand{\mbw}{\mb{w}}
\newcommand{\mbW}{\mb{W}}

\newcommand{\mbx}{\mb{x}}
\newcommand{\mbX}{\mb{X}}

\newcommand{\mby}{\mb{y}}
\newcommand{\mbY}{\mb{Y}}

\newcommand{\mbz}{\mb{z}}
\newcommand{\mbZ}{\mb{Z}}
\newcommand{\mbT}{\mb{T}}
\newcommand{\mbA}{\mb{A}}
\newcommand{\mba}{\mb{a}}

\newcommand{\mbI}{\mb{I}}
\newcommand{\mbone}{\mb{1}}

\newcommand{\mbL}{\mb{L}}

\newcommand{\mbtheta}{\mb{\theta}}
\newcommand{\mbTheta}{\mb{\Theta}}
\newcommand{\mbomega}{\mb{\omega}}
\newcommand{\mbOmega}{\mb{\Omega}}
\newcommand{\mbsigma}{\mb{\sigma}}
\newcommand{\mbSigma}{\mb{\Sigma}}
\newcommand{\mbphi}{\mb{\phi}}
\newcommand{\mbPhi}{\mb{\Phi}}

\newcommand{\mbalpha}{\mb{\alpha}}
\newcommand{\mbbeta}{\mb{\beta}}
\newcommand{\mbgamma}{\mb{\gamma}}
\newcommand{\mbeta}{\mb{\eta}}
\newcommand{\mbmu}{\mb{\mu}}
\newcommand{\mbrho}{\mb{\rho}}
\newcommand{\mblambda}{\mb{\lambda}}
\newcommand{\mbzeta}{\mb{\zeta}}

\newcommand\dif{\mathop{}\!\mathrm{d}}
\newcommand{\diag}{\textrm{diag}}
\newcommand{\supp}{\textrm{supp}}

\newcommand{\V}{\mathbb{V}}
\newcommand{\bbH}{\mathbb{H}}

\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbZ}{\mathbb{Z}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbS}{\mathbb{S}}

\newcommand{\cL}{\mathcal{L}}
\newcommand{\cD}{\mathcal{D}}

\newcommand{\cN}{\mathcal{N}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\Gam}{\textrm{Gam}}
\newcommand{\InvGam}{\textrm{InvGam}}

% \newcommand{\qedsymbol}{\rule{0.7em}{0.7em}}

\newcommand{\g}{\, | \,}
\newcommand{\s}{\, ; \,}

\def\checkmark{\tikz\fill[scale=0.4](0,.35) -- (.25,0) -- (1,.7) -- (.25,.15) -- cycle;} 


\usepackage{booktabs,arydshln}
\makeatletter
\def\adl@drawiv#1#2#3{%
        \hskip.5\tabcolsep
        \xleaders#3{#2.5\@tempdimb #1{1}#2.5\@tempdimb}%
                #2\z@ plus1fil minus1fil\relax
        \hskip.5\tabcolsep}
\newcommand{\cdashlinelr}[1]{%
  \noalign{\vskip\aboverulesep
           \global\let\@dashdrawstore\adl@draw
           \global\let\adl@draw\adl@drawiv}
  \cdashline{#1}
  \noalign{\global\let\adl@draw\@dashdrawstore
           \vskip\belowrulesep}}
\makeatother

\newenvironment{proofsk}{%
  \renewcommand{\proofname}{Proof sketch}\proof}{\endproof}

\renewcommand{\epsilon}{\varepsilon}

%********************************************************************
% Extra theorem environments
%********************************************************************

\declaretheorem[style=plain,numberwithin=section,name=Theorem]{theorem}
\declaretheorem[style=plain,sibling=theorem,name=Lemma]{lemma}
\declaretheorem[style=plain,sibling=theorem,name=Proposition]{proposition}
\declaretheorem[style=plain,sibling=theorem,name=Corollary]{corollary}
\declaretheorem[style=plain,sibling=theorem,name=Claim]{claim}
\declaretheorem[style=plain,sibling=theorem,name=Conjecture]{conjecture}
\declaretheorem[style=definition,sibling=theorem,name=Definition]{definition}
\declaretheorem[style=definition,name=Assumption]{assumption}
\declaretheorem[style=definition,sibling=theorem,name=Example]{example}
\declaretheorem[style=remark,sibling=theorem,name=Remark]{remark}

\newenvironment{example*}
 {\pushQED{\qed}\example}
 {\popQED\endexample}
\numberwithin{equation}{section}


==> preamble/commenting.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% EDITING HELPER FUNCTIONS  %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% NA: needs attention (rough writing whose correctness needs to be verified)
%% TBD: instructions for how to fix a gap ("Describe the propagation by ...")
%% PROBLEM: bug or missing crucial bit 

%% use \fXXX versions of these macros to put additional explanation into a footnote.  
%% The idea is that we don't want to interrupt the flow of the paper or make it 
%% impossible to read because there are a bunch of comments.

%% NA's (and TBDs, those less crucially) should be written so 
%% that they flow with the text.

\definecolor{WowColor}{rgb}{.75,0,.75}
\definecolor{SubtleColor}{rgb}{0,0,.50}

% inline
\newcommand{\NA}[1]{\textcolor{SubtleColor}{ {\tiny \bf ($\star$)} #1}}
\newcommand{\LATER}[1]{\textcolor{SubtleColor}{ {\tiny \bf ($\dagger$)} #1}}
\newcommand{\TBD}[1]{\textcolor{SubtleColor}{ {\tiny \bf (!)} #1}}
\newcommand{\PROBLEM}[1]{\textcolor{WowColor}{ {\bf (!!)} {\bf #1}}}

% as margin notes

\newcounter{margincounter}
\newcommand{\displaycounter}{{\arabic{margincounter}}}
\newcommand{\incdisplaycounter}{{\stepcounter{margincounter}\arabic{margincounter}}}

\newcommand{\fTBD}[1]{\textcolor{SubtleColor}{$\,^{(\incdisplaycounter)}$}\marginpar{\tiny\textcolor{SubtleColor}{ {\tiny $(\displaycounter)$} #1}}}

\newcommand{\fPROBLEM}[1]{\textcolor{WowColor}{$\,^{((\incdisplaycounter))}$}\marginpar{\tiny\textcolor{WowColor}{ {\bf $\mathbf{((\displaycounter))}$} {\bf #1}}}}

\newcommand{\fLATER}[1]{\textcolor{SubtleColor}{$\,^{(\incdisplaycounter\dagger)}$}\marginpar{\tiny\textcolor{SubtleColor}{ {\tiny $(\displaycounter\dagger)$} #1}}}


==> preamble/nocommenting.tex <==
\newcommand{\LATER}[1]{\error}
\newcommand{\fLATER}[1]{\error}
\newcommand{\TBD}[1]{\error}
\newcommand{\fTBD}[1]{}
\newcommand{\PROBLEM}[1]{\error}
\newcommand{\fPROBLEM}[1]{\error}
\newcommand{\NA}[1]{#1} 

